An accurate solar axions ray-tracing response of BabyIAXO

BabyIAXO is the intermediate stage of the International Axion Observatory (IAXO) to be hosted at DESY. Its primary goal is the detection of solar axions following the axion helioscope technique. Axions are converted into photons in a large magnet that is pointing to the sun. The resulting X-rays are focused by appropriate X-ray optics and detected by sensitive low-background detectors placed at the focal spot. The aim of this article is to provide an accurate quantitative description of the different components (such as the magnet, optics, and X-ray detectors) involved in the detection of axions. Our efforts have focused on developing robust and integrated software tools to model these helioscope components, enabling future assessments of modifications or upgrades to any part of the IAXO axion helioscope and evaluating the potential impact on the experiment's sensitivity. In this manuscript, we demonstrate the application of these tools by presenting a precise signal calculation and response analysis of BabyIAXO's sensitivity to the axion-photon coupling. Though focusing on the Primakoff solar flux component, our virtual helioscope model can be used to test different production mechanisms, allowing for direct comparisons within a unified framework.

==> include/connections.tex <==
\begin{tikzpicture}
	\node[align=center] (sol) at (0,0) {Solar\\model};
	\node[right=of sol, align=center] (op) {Opacity\\code};
	\node (mid1) at ($(sol)!0.5!(op)$) {};
	\node[iq, below=of mid1] (flux) {Solar axion flux};
	\node[iq, below right=of mid1, xshift=1.5cm] (eff) {Instr.\ resp.};
	\node[right=of op, xshift=-0.5cm] (ergres) {$\Delta E$};
	\node[right=of ergres] (effo) {$\epsilon_\text{opt}$};
	\node[right=of effo] (effd) {$\epsilon_\text{det}$};
	\node[right=of effd] (effb) {$\epsilon_B$};
	\node[right=of effb] (efft) {$\epsilon_\text{t}$};
	\node (mid2) at ($(flux)!0.5!(eff)$) {};
	\node[sq, below=of mid2] (sig) {Signal $s$};
	\node[draw, circle] (ast) at ($(mid2)!0.3!(sig)$) {$\ast$};
	\node[draw, rectangle, rounded corners, right=of sig] (loglike) {$\log(L)$};
	\node[sq, above right=of loglike] (bkg) {Bkg $b$};
	\node[right=of bkg, yshift=0.5cm] (bd) {$b_\text{dark}$};
	\node[below=of bd] (bn) {$b_\text{therm}$};
	\node[sq, right= of loglike] (data) {Data $n$};
	
	\draw (sol) -- (flux);
	\draw (op) -- (flux);
	\draw (eff) -- (ast) (flux) -- (ast) -- (sig);
	\draw (ergres) -- (eff);
	\draw (effo) -- (eff);
	\draw (effd) -- (eff);
	\draw (effb) -- (eff);
	\draw (efft) -- (eff);
	\draw (bd) -- (bkg);
	\draw (bn) -- (bkg);
	\draw (sig) -- (loglike);
	\draw (bkg) -- (loglike);
	\draw (data) -- (loglike);
\end{tikzpicture}

==> sections/backup.tex <==
The Sun is a natural source of ALPs. 
These can be produced through a variety of mechanisms, depending on their couplings with SM fields. 
The most relevant production mechanism associated with the axion-photon coupling ($g_{a\gamma}$) is the Primakoff process, 
in which ALPs are converted into ALPs in the electrons and ions electric field $\gamma + Ze \to Ze+a$. 
The axion-photon coupling would also trigger photon-ALPs conversions in macroscopic fields inside the sun. 
As we shall see, this contribution is subject to uncertainties due to the structure and exact intensity of the magnetic field, whereas the Primakoff contribution depends only on very well understood properties of the sun, particularly its temperature profile. 

The most significant production mechanisms in the case of ALPs coupled with electrons are Atomic recombination and de-excitation, the electron and ion Bremsstrahlung, and the Compton process, collectively known as the ABC processes~\cite{Redondo:2013wwa} .\footnote{An additional  astrophysical process is the electron-positron annihilation, $ e^{+} e^{-} \to \gamma + a $~\cite{Pantziris:1986dc}. 
However, this process is highly suppressed in the solar core since the temperature is significantly lower than the positron mass and so the positron population is very suppressed.}

Finally, axions coupled to nucleons can be produced through nuclear processes.
There are two noteworthy mechanisms for this: nuclear fusion and decays as well as thermal excitation and subsequent de-excitation of the nuclei of stable isotopes.  
There an enormous number of nuclear reactions that produce axions.
However, in most cases the axion flux is expected to be extremely small. 
The axion production mechanisms that are most relevant in the sun are the following:
Proton-deuterium fusion reaction, $p+d\to$ $^{3}{\rm He}+a$\,(5.5\,MeV); 
Lithium de-excitation $^7{\rm Li}^* \to\, ^7{\rm Li}+a\,({\rm 0.478\,MeV})$;
$^{57}$Fe de-excitation, $^{57}{\rm Fe}^* \to\, ^{57}{\rm Fe}+a\,({\rm 144\,keV})$~\cite{Moriyama:1995bz,Krcmar:1998xn}.
Of the above processes, the most relevant is perhaps the latest.
Notice that the fluxes above depend of combinations of the couplings with protons and neutrons which are specific of each process.

In genera, therefore, we expect to observe solar axions on Earth with a spectrum 
%
\begin{align}
\label{eq:solar_flux_1}
\frac{dN_a}{dt d\omega}
=\left( \frac{g_{a\gamma}}{{\rm GeV}^{-1}} \right)^{2}\,n_{a\gamma}(\omega) +g_{ae}^2\,n_{ae}(\omega) 
+ g_{ap}^2\,n_{ap}(\omega) + g_{an}^2\,n_{an}(\omega) 
\,,
\end{align}
%
where $n_{ai}$ represent the contributions from processes induced by the different axion couplings. 
Good analytical approximations for these coefficients exist for all but the atomic recombination and deexcitation processes (see, e.g., Ref.~\cite{Andriamonje:2007ew} and \cite{Barth:2013sma}):
%
\begin{subequations}\label{eq:solar_flux_approx}
\begin{align}
&n_{a\gamma}(\omega)\approx
1.69\times 10^{58}
e^{-0.829 \,\omega}\omega^{2.45}
\,{\rm keV}^{-1}{\rm s}^{-1}\,; \\
& n_{ae}^{B}\approx 7.4\times 10^{62}
\frac{\omega\,e^{-0.77\,\omega}}{1+0.667\,\omega^{1.278}}
\,{\rm keV}^{-1}{\rm s}^{-1}\,; \\
& n_{ae}^{C}\approx 3.7\times 10^{60}
\omega^{2.987}\,e^{-0.776\,\omega}
\,{\rm keV}^{-1}{\rm s}^{-1} \,.
\end{align}
\end{subequations}
%
The total number of axions emitted by the Sun per second through Primakoff and ABC processes is,
%%
%\begin{align}\label{eq:solar_spectrum_integrated}
%\frac{dN_a}{dt}
%=1.1\times 10^{39} \,{\rm s}^{-1} 
%\left( \,g_{\gamma 10}^{2} \,{\rm s}^{-1} + 0.7\,g_{e 12}^{2} \right)  \,.
%\end{align}
%%
%
\begin{align}\label{eq:solar_spectrum_integrated}
\frac{dN_a}{dt}
=1.1\times 10^{39} 
\left[ 
\left( 
\frac{g_{a\gamma}}{10^{-10}{\rm GeV}^{-1}} 
\right)^2  
+ 0.7\,
\left( 
\frac{g_{ae}}{10^{-12}} 
\right)^{2} 
\right] \,{\rm s}^{-1}  \,.
\end{align}
%
%where $g_{\gamma 10}=g_{a\gamma}/10^{-10}{\rm GeV}^{-1}$ and $g_{e 12}=g_{ae}/10^{-12}$.
%
\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.45\linewidth]{figures/fig_solar_flux.pdf}
		\caption{Solar axion spectrum from Primakoff and ABC processes. 
}
		\label{fig_solar_flux}
	\end{center}
\end{figure}
%
Evidently, the axion flux gets a similar contribution from Primakoff and ABC axions for couplings of phenomenological interest (cf.~\ref{fig_solar_flux}).
Notice, however, that the ABC flux is peaked at slightly lower energies than the Primakoff, a fact that allows to distinguish between the two fluxes (and so infer some information about the underlying axion model) if enough data is collected in an helioscope experiment~\cite{Jaeckel:2018mbn}.\footnote{For example, the number of axions produced in the energy bin $1\leq \omega/{\rm keV}\leq 2$ is 12.5\% of the total, in the case of hadronic axions (no coupling with electrons) but it moves quickly to $\sim 30\%$ if $g_{ae}/g_{a\gamma}>5\times 10^{-2}\,{\rm GeV}$, which is typical for DFSZ axions. }

The weight of the two contributions in \eqref{eq:solar_spectrum_integrated} depends on the specific axion model.
%To estimate the experimental potential it is convenient to introduce the model-dependent ratio 
%%
%\begin{align}
%\xi=C_e/C_{\gamma}\,.
%\end{align}
%%
In terms of 
$g_{e 12}=g_{ae}/10^{-12}$
and  $g_{\gamma 10}=g_{a\gamma}/10^{-10}{\rm GeV}^{-1}$, we have
%
\begin{subequations}
\label{eq:ge12gg10}
\begin{align}
& {\rm KSVZ}:  ~ ~\,~ g_{e12}/g_{\gamma 10} \approx 0\,; \\
& {\rm DFSZ~I}:  ~~g_{e12}/g_{\gamma 10}  = 20 \sin^{2}\beta\,;  \\
& {\rm DFSZ~II}:  ~g_{e12}/g_{\gamma 10} = 12 \cos^{2}\beta\,.
\end{align}
\end{subequations}
%
